TOP-ERL: Transformer-based Off-Policy Episodic Reinforcement Learning

This work introduces Transformer-based Off-Policy Episodic Reinforcement Learning (TOP-ERL), a novel algorithm that enables off-policy updates in the ERL framework. In ERL, policies predict entire action trajectories over multiple time steps instead of single actions at every time step. These trajectories are typically parameterized by trajectory generators such as Movement Primitives (MP), allowing for smooth and efficient exploration over long horizons while capturing high-level temporal correlations. However, ERL methods are often constrained to on-policy frameworks due to the difficulty of evaluating state-action values for entire action sequences, limiting their sample efficiency and preventing the use of more efficient off-policy architectures. TOP-ERL addresses this shortcoming by segmenting long action sequences and estimating the state-action values for each segment using a transformer-based critic architecture alongside an n-step return estimation. These contributions result in efficient and stable training that is reflected in the empirical results conducted on sophisticated robot learning environments. TOP-ERL significantly outperforms state-of-the-art RL methods. Thorough ablation studies additionally show the impact of key design choices on the model performance.

==> figure_and_table/ablation_no_target/__all_no_target__.tex <==
\begin{figure}[h]
    % \hspace{-2mm}
    \centering    
    \vspace{4mm}
    \begin{minipage}[t]{0.24\textwidth}
        \resizebox{\textwidth}{!}{        
        \input{figure_and_table/ablation_no_target/ablation_no_target}}%       
    \end{minipage}
    \begin{minipage}[t]{0.22\textwidth}
        \vspace{-2.7cm} % Move the legend up by 2cm        
        \resizebox{\textwidth}{!}{                
        \input{figure_and_table/ablation_no_target/legend_no_target}}        
    \end{minipage}
    \caption{\centering With target net or not}
    \label{fig:ablation_no_target}
    \vspace{-4mm}
\end{figure}

==> figure_and_table/ablation_no_target/ablation_no_target.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%           Box Dense num_segments Ablation
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




    % \addlegendimage{C0, line width=\linewidthtcp}
    % \addlegendentry{Random};          
    % \addlegendimage{C9, line width=\linewidthothers}
    % \addlegendentry{1 Seg.};    
    % \addlegendimage{C1, line width=\linewidthothers}
    % \addlegendentry{2 Seg.};    
    % \addlegendimage{C3, line width=\linewidthothers}
    % \addlegendentry{5 Seg.};    
    % \addlegendimage{C4, line width=\linewidthothers}
    % \addlegendentry{10 Seg.};    
    % \addlegendimage{C6, line width=\linewidthothers}
    % \addlegendentry{25 Seg.};  

% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}
\def\top_color{C0}
\def\segone_color{C9}
\def\segtwo_color{C4}
\def\segfive_color{C3}
\def\segten_color{C1}
\def\segtwentyfive_color{C6}
\def\linewidthtop{1mm}
\def\linewidthothers{0.5mm}


\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204, at={(0.03,0.03)},  anchor=north west},
% title={Box Pushing - Dense},
% every x tick scale label/.style={
%     at={(1,0)},yshift=5pt, xshift=-5pt,anchor=south east,inner sep=0pt
% },
tick align=outside,
tick pos=left,
% x grid style={darkgray176},
x grid style={white},
scaled x ticks=false,
xticklabels={,0,2,4,6,8,10},
% xticklabels={,0,0.5,1,1.5,2, 2.5, 3},
xlabel={Environment Interactions ($\times 10^6$)},
xmajorgrids,
% xmin=-2500000, xmax=42000000.05,
% xmin=-1500000, xmax=31000000.05,
xmin=-300000, xmax=10200000.05,
% xmin=-1500000, xmax=101000000.05,
xtick style={color=black},
% y grid style={darkgray176},
y grid style={white},
ylabel={Success Rate, IQM},
ymajorgrids,
ymin=-0.05, ymax=0.90,
ytick style={color=black},
axis background/.style={fill=plot_background},
label style={font=\large},
tick label style={font=\large},
x axis line style={draw=none},
y axis line style={draw=none},
]


% %%%%%%%%%%%%%%%%%%%% Seg 10 %%%%%%%%%%%%%%%%%%%
\path [draw=\segten_color, fill=\segten_color, opacity=0.2]
(axis cs:51600,0)
--(axis cs:51600,0)
--(axis cs:51600,0)
--(axis cs:451600,0)
--(axis cs:451600,0)
--(axis cs:851600,0)
--(axis cs:851600,0)
--(axis cs:1251600,0)
--(axis cs:1251600,0)
--(axis cs:1651600,0.00736778664494864)
--(axis cs:1651600,0.00739007252263946)
--(axis cs:2051600,0.0155173522960431)
--(axis cs:2451600,0.0213009161697567)
--(axis cs:2451600,0.0213009161697567)
--(axis cs:2851600,0.0347209514977891)
--(axis cs:2851600,0.0347209514977891)
--(axis cs:3251600,0.0527185945359647)
--(axis cs:3251600,0.0531459016926456)
--(axis cs:3651600,0.059618426856644)
--(axis cs:3651600,0.0583324438597825)
--(axis cs:4051600,0.107397967777538)
--(axis cs:4451600,0.110777218928955)
--(axis cs:4451600,0.111024182181889)
--(axis cs:4851600,0.129858738189605)
--(axis cs:4851600,0.130070947799716)
--(axis cs:5251600,0.139344820667913)
--(axis cs:5251600,0.138105434655565)
--(axis cs:5651600,0.156561225092696)
--(axis cs:5651600,0.156167726538405)
--(axis cs:6051600,0.173654385557647)
--(axis cs:6051600,0.173468718763152)
--(axis cs:6451600,0.164718555508207)
--(axis cs:6851600,0.172484050484553)
--(axis cs:6851600,0.17458815121624)
--(axis cs:7251600,0.215766714873882)
--(axis cs:7251600,0.212566652250747)
--(axis cs:7651600,0.200975022541669)
--(axis cs:7651600,0.201867511218658)
--(axis cs:8051600,0.201511221003065)
--(axis cs:8051600,0.2013751608701)
--(axis cs:8451600,0.186254435089719)
--(axis cs:8851600,0.172397400005922)
--(axis cs:8851600,0.172397400005922)
--(axis cs:9251600,0.185415763120389)
--(axis cs:9251600,0.185212468363173)
--(axis cs:9651600,0.1554848872502)
--(axis cs:9651600,0.1554848872502)
--(axis cs:10051600,0.154973154245556)
--(axis cs:10051600,0.155806968518928)
--(axis cs:10451600,0.184829775968076)
% --(axis cs:10851600,0.167322956937156)
% --(axis cs:10851600,0.244149438481994)
% --(axis cs:10851600,0.244149438481994)
--(axis cs:10451600,0.236729764025407)
--(axis cs:10051600,0.240853895458705)
--(axis cs:10051600,0.240134591950119)
--(axis cs:9651600,0.237275809387145)
--(axis cs:9651600,0.236640490965399)
--(axis cs:9251600,0.292620675811974)
--(axis cs:9251600,0.289319625573037)
--(axis cs:8851600,0.26528443297021)
--(axis cs:8851600,0.26528443297021)
--(axis cs:8451600,0.271651727736397)
--(axis cs:8051600,0.28285923094159)
--(axis cs:8051600,0.284059424554455)
--(axis cs:7651600,0.290976210568749)
--(axis cs:7651600,0.290976210568749)
--(axis cs:7251600,0.281765665944098)
--(axis cs:7251600,0.282472507190021)
--(axis cs:6851600,0.246314054679219)
--(axis cs:6851600,0.245406928775628)
--(axis cs:6451600,0.22697633952431)
--(axis cs:6051600,0.227465198295957)
--(axis cs:6051600,0.227465198295957)
--(axis cs:5651600,0.205233911323067)
--(axis cs:5651600,0.206063806359469)
--(axis cs:5251600,0.205127949928656)
--(axis cs:5251600,0.203860769578558)
--(axis cs:4851600,0.203417656633818)
--(axis cs:4851600,0.20398062878323)
--(axis cs:4451600,0.162822186613468)
--(axis cs:4451600,0.162090815271356)
--(axis cs:4051600,0.159593549854468)
--(axis cs:3651600,0.105383379115011)
--(axis cs:3651600,0.105306273198064)
--(axis cs:3251600,0.0782392150452326)
--(axis cs:3251600,0.0782472905307913)
--(axis cs:2851600,0.0547131626444078)
--(axis cs:2851600,0.0536928533030599)
--(axis cs:2451600,0.0439911384478325)
--(axis cs:2451600,0.0431171446708448)
--(axis cs:2051600,0.0325329312396725)
--(axis cs:1651600,0.0140300550458505)
--(axis cs:1651600,0.0139376590619178)
--(axis cs:1251600,0.0026726973883342)
--(axis cs:1251600,0.0026726973883342)
--(axis cs:851600,0)
--(axis cs:851600,0)
--(axis cs:451600,0)
--(axis cs:451600,0)
--(axis cs:51600,0)
--(axis cs:51600,0)
--cycle;

\addplot [line width=\linewidthothers, \segten_color, mark=*, mark size=0, mark options={solid}]
table {%
51600 0
51600 0
451600 0
451600 0
851600 0
851600 0
1251600 0
1251600 0
1651600 0.00931830162164715
1651600 0.00931830162164715
2051600 0.0233041023331343
2451600 0.0330813171642899
2451600 0.0330813171642899
2851600 0.0463466918658862
2851600 0.0463466918658862
3251600 0.0639907768886466
3251600 0.0639907768886466
3651600 0.0846893412995047
3651600 0.0846893412995047
4051600 0.135707640210785
4451600 0.134396284676984
4451600 0.134396284676984
4851600 0.163662898788404
4851600 0.163662898788404
5251600 0.170529764328216
5251600 0.170529764328216
5651600 0.171310717713091
5651600 0.171310717713091
6051600 0.18989517067665
6051600 0.18989517067665
6451600 0.193983604414777
6851600 0.218863946139418
6851600 0.218863946139418
7251600 0.246388058714785
7251600 0.246388058714785
7651600 0.237071330813335
7651600 0.237071330813335
8051600 0.247192700256924
8051600 0.247192700256924
8451600 0.234554497635502
8851600 0.228762758107652
8851600 0.228762758107652
9251600 0.253461475830731
9251600 0.253461475830731
9651600 0.211916032105112
9651600 0.211916032105112
10051600 0.210559256738575
10051600 0.210559256738575
% 10451600 0.210367880452971
% 10851600 0.206157037259593
};



%%%%%%%%%%%%%%%%%%%%%%%%%%   TOP-ERL (V-target) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path [draw=\top_color, fill=\top_color, opacity=0.2]
(axis cs:51600,0)
--(axis cs:51600,0)
--(axis cs:51600,0)
--(axis cs:451600,0)
--(axis cs:851600,0)
--(axis cs:851600,0)
--(axis cs:1251600,0)
--(axis cs:1651600,0.0131466512618772)
--(axis cs:1651600,0.0133353784493693)
--(axis cs:2051600,0.0413283457609199)
--(axis cs:2451600,0.151337953148107)
--(axis cs:2451600,0.153033561316605)
--(axis cs:2851600,0.218478743107844)
--(axis cs:3251600,0.397638408343607)
--(axis cs:3651600,0.536365572746305)
--(axis cs:3651600,0.536365572746305)
--(axis cs:4051600,0.542737674887022)
--(axis cs:4451600,0.634593733450746)
--(axis cs:4451600,0.634350496225742)
--(axis cs:4851600,0.670431850454353)
--(axis cs:5251600,0.69874036762053)
--(axis cs:5251600,0.69874036762053)
--(axis cs:5651600,0.706190630635517)
--(axis cs:6051600,0.723602532536877)
--(axis cs:6051600,0.722043680587771)
--(axis cs:6451600,0.709640033945828)
--(axis cs:6851600,0.729547517908204)
--(axis cs:7251600,0.75241802071214)
--(axis cs:7251600,0.754133556943073)
--(axis cs:7651600,0.726270778715126)
--(axis cs:8051600,0.745617934845087)
--(axis cs:8051600,0.747517433998734)
--(axis cs:8451600,0.757970219585967)
--(axis cs:8851600,0.752786080029104)
--(axis cs:8851600,0.752652607507845)
--(axis cs:9251600,0.762163220737448)
--(axis cs:9651600,0.745403143231365)
--(axis cs:9651600,0.745403143231365)
--(axis cs:10051600,0.766988262380617)
--(axis cs:10451600,0.789557954141376)
% --(axis cs:10851600,0.796397797038731)
% --(axis cs:10851600,0.795766582873564)
% --(axis cs:11251600,0.797460649066761)
% --(axis cs:11651600,0.793669734897496)
% --(axis cs:11651600,0.793669734897496)
% --(axis cs:12051600,0.806029208578972)
% --(axis cs:12451600,0.795611930110023)
% --(axis cs:12451600,0.796433357463573)
% --(axis cs:12851600,0.818325637972671)
% --(axis cs:13251600,0.796575162493517)
% --(axis cs:13651600,0.804022423018633)
% --(axis cs:13651600,0.844284141166215)
% --(axis cs:13651600,0.844284141166215)
% --(axis cs:13251600,0.824133676298188)
% --(axis cs:12851600,0.841635612772295)
% --(axis cs:12451600,0.838010073446124)
% --(axis cs:12451600,0.837020047576055)
% --(axis cs:12051600,0.846495495401783)
% --(axis cs:11651600,0.821969635370778)
% --(axis cs:11651600,0.822210457329349)
% --(axis cs:11251600,0.833426236247573)
% --(axis cs:10851600,0.841770976709186)
% --(axis cs:10851600,0.841870068643878)
--(axis cs:10451600,0.816459918375224)
--(axis cs:10051600,0.80394763777913)
--(axis cs:9651600,0.798299079016656)
--(axis cs:9651600,0.797390752585934)
--(axis cs:9251600,0.789059949039621)
--(axis cs:8851600,0.790170416601394)
--(axis cs:8851600,0.790170416601394)
--(axis cs:8451600,0.790510777667517)
--(axis cs:8051600,0.789694565549258)
--(axis cs:8051600,0.789156479071252)
--(axis cs:7651600,0.779193028472285)
--(axis cs:7251600,0.787149462163176)
--(axis cs:7251600,0.787199014537395)
--(axis cs:6851600,0.759500270669563)
--(axis cs:6451600,0.767282983455012)
--(axis cs:6051600,0.752269109179855)
--(axis cs:6051600,0.752269109179855)
--(axis cs:5651600,0.729397499479084)
--(axis cs:5251600,0.735074605739488)
--(axis cs:5251600,0.735074605739488)
--(axis cs:4851600,0.731183334981695)
--(axis cs:4451600,0.698317217312372)
--(axis cs:4451600,0.698317217312372)
--(axis cs:4051600,0.649858462978944)
--(axis cs:3651600,0.566052867595783)
--(axis cs:3651600,0.565478845735699)
--(axis cs:3251600,0.449718964194615)
--(axis cs:2851600,0.374733433743337)
--(axis cs:2451600,0.21567838168538)
--(axis cs:2451600,0.21567838168538)
--(axis cs:2051600,0.0886873339425088)
--(axis cs:1651600,0.0291607500566329)
--(axis cs:1651600,0.029213754257114)
--(axis cs:1251600,0.00123355264076963)
--(axis cs:851600,0)
--(axis cs:851600,0)
--(axis cs:451600,0)
--(axis cs:51600,0)
--(axis cs:51600,0)
--cycle;

\addplot [line width=\linewidthtop, \top_color, mark=*, mark size=0, mark options={solid}]
table {%
51600 0
51600 0
451600 0
851600 0
851600 0
1251600 0
1651600 0.0220152198515962
1651600 0.0220152198515962
2051600 0.070129991957565
2451600 0.190895397608125
2451600 0.190895397608125
2851600 0.309443728996178
3251600 0.425461189570063
3651600 0.552733510780102
3651600 0.552733510780102
4051600 0.610597546232128
4451600 0.684460573981626
4451600 0.684460573981626
4851600 0.70768100869192
5251600 0.720824015807427
5251600 0.720824015807427
5651600 0.712405588903529
6051600 0.742159905932434
6051600 0.742159905932434
6451600 0.752815203159023
6851600 0.7430671579336
7251600 0.7755493257093
7251600 0.7755493257093
7651600 0.762378863556387
8051600 0.772692377007164
8051600 0.772692377007164
8451600 0.774128291362219
8851600 0.770276302722307
8851600 0.770276302722307
9251600 0.772789142627761
9651600 0.779565297859506
9651600 0.779565297859506
10051600 0.779899904310781
10451600 0.802167711280924
% 10851600 0.825507342138272
% 10851600 0.825507342138272
% 11251600 0.825152272030602
% 11651600 0.811417314320251
% 11651600 0.811417314320251
% 12051600 0.825187306397627
% 12451600 0.817418673935725
% 12451600 0.817418673935725
% 12851600 0.830139957000396
% 13251600 0.811123270110975
% 13651600 0.829344004601192
};



\end{axis}
\end{tikzpicture}

==> figure_and_table/ablation_no_target/legend_no_target.tex <==
\begin{tikzpicture} 
\def\linewidthtcp{1mm}
\def\linewidthothers{0.5mm}

    \begin{axis}[%
    hide axis,
    xmin=10,
    xmax=50,
    ymin=0,
    ymax=0.4,
    legend style={
        draw=white!15!black,
        legend cell align=left,
        legend columns=1, 
        legend style={
            draw=none,
            column sep=1ex,
            line width=1pt,            
        }
    },
    ]
    \addlegendimage{C0, line width=\linewidthtcp}
    \addlegendentry{With Target Net};          
    % \addlegendimage{C9, line width=\linewidthothers}
    % \addlegendentry{100\%.};    
    % \addlegendimage{C4, line width=\linewidthothers}
    % \addlegendentry{50\%.};    
    % \addlegendimage{C3, line width=\linewidthothers}
    % \addlegendentry{20\%};    
    \addlegendimage{C1, line width=\linewidthothers}
    \addlegendentry{Without Target Net};    
    % \addlegendimage{C6, line width=\linewidthothers}
    % \addlegendentry{5\%};    
    

    
    % Use dashed lines for the num of segment ablation?        
    \end{axis}
\end{tikzpicture}

==> figure_and_table/abltion_transformer/__all_critic_transformer__.tex <==
\begin{figure}[h]
    % \hspace{-2mm}
    \centering    
    \vspace{4mm}
    \begin{minipage}[t]{0.24\textwidth}
        \resizebox{\textwidth}{!}{                \input{figure_and_table/abltion_transformer/ablation_critic_transformer}}%       
    \end{minipage}
    \begin{minipage}[t]{0.25\textwidth}
        \vspace{-2.7cm} % Move the legend up by 2cm        
        \resizebox{\textwidth}{!}{                
        \input{figure_and_table/abltion_transformer/legend_critic_transformer}}        
    \end{minipage}
    \caption{\centering Demonstrate the effectiveness of critic transformer}
    \label{fig:ablation_transformer}
    % \vspace{-4mm}
\end{figure}

==> figure_and_table/abltion_transformer/__all_target_bias__.tex <==
\begin{figure}[h]
    % \hspace{-2mm}
    \centering    
    \vspace{4mm}
    \begin{minipage}[h]{0.42\textwidth}
        \resizebox{\textwidth}{!}{                \input{figure_and_table/abltion_transformer/value_bias}}%       
    \end{minipage}
    \begin{minipage}[t]{0.28\textwidth}
        \vspace{-2.7cm} % Move the legend up by 2cm        
        \resizebox{\textwidth}{!}{                
        \input{figure_and_table/abltion_transformer/legend_target_bias}}      
    \end{minipage}
    % \begin{minipage}[t]{0.34\textwidth}
    %     \resizebox{\textwidth}{!}{                \input{figure_and_table/abltion_transformer/target_bias}}%       
    % \end{minipage}
    \caption{Comparison of critic bias between TOP-ERL and its ablated version. The results are reported starting from 2M environment interactions (corresponding to 1.2M steps since the policy training begins). }
    \label{fig:ablation_value_bias}
    % \vspace{-4mm}
\end{figure}

==> figure_and_table/abltion_transformer/__all_value_error__.tex <==
\begin{figure}[h]
    % \hspace{-2mm}
    \centering    
    \vspace{4mm}
    \begin{minipage}[t]{0.44\textwidth}
        \resizebox{\textwidth}{!}{                \input{figure_and_table/abltion_transformer/critic_error}}%       
    \end{minipage}
    % \begin{minipage}[t]{0.24\textwidth}
    %     \resizebox{\textwidth}{!}{                \input{figure_and_table/abltion_transformer/critic_error_4to10M}}%   
    % \end{minipage}
    \begin{minipage}[t]{0.44\textwidth}
        \vspace{-4.7cm} % Move the legend up by 2cm        
        \resizebox{\textwidth}{!}{                
        \input{figure_and_table/abltion_transformer/legend_error}}        
    \end{minipage}
    \caption{Comparison of average critic predictions and average Monte Carlo True returns across TOP-ERL and its ablated version. The analysis methodology is consistent with the approach discussed in Clipped Double Q-learning \citep{fujimoto2018addressing}. The steps before 0.8M represent the warm-up phase of the critic network, where the policy net was not trained. }
    \label{fig:ablation_critic_value}
    % \vspace{-4mm}
\end{figure}

==> figure_and_table/box_pushing_40M/__all40M__.tex <==
\begin{figure}[h]
    \centering
    \hspace*{\fill}%
    \resizebox{0.9\textwidth}{!}{
        \input{figure_and_table/emprical_result/legend}
    }%  
    \hspace*{\fill}%
    \newline    
    \hspace*{\fill}%
    \begin{subfigure}{0.24\textwidth}        
        \resizebox{\textwidth}{!}{\input{figure_and_table/box_pushing_40M/box_dense_40M}}%
        \caption{\centering Box Pushing \\~~~~~~~~Dense Reward}
        \label{subfig:hopper_height_40m}
    \end{subfigure}
    \hfill       
    \begin{subfigure}{0.24\textwidth}
        \resizebox{\textwidth}{!}{\input{figure_and_table/box_pushing_40M/box_sparse_40M}}%
        \caption{\centering Box Pushing \\~~~~~~~~~Sparse Reward}
        \label{subfig:bp_dense_success_40m}
    \end{subfigure}
    \hspace*{\fill}%        
    \caption{Continue training TOP-ERL till 40M.}
    \label{fig:bp_40m}
    % \vspace{-0.3cm}
\end{figure}
% \vspace{-1cm}

==> figure_and_table/box_pushing_40M/legend.tex <==
\begin{tikzpicture} 
\def\linewidthtcp{1mm}
\def\linewidthothers{0.5mm}

    \begin{axis}[%
    hide axis,
    xmin=10,
    xmax=50,
    ymin=0,
    ymax=0.4,
    legend style={
        draw=white!15!black,
        legend cell align=left,
        legend columns=-1, 
        legend style={
            draw=none,
            column sep=1ex,
            line width=1pt
        }
    },
    ]
    \addlegendimage{C0, line width=\linewidthtcp}
    \addlegendentry{\mname (ours)};    
    \addlegendimage{C1, line width=\linewidthothers}
    \addlegendentry{\acrshort{tcp}};
    \addlegendimage{C9, line width=\linewidthothers}
    \addlegendentry{\acrshort{bbrl}};
    \addlegendimage{C2, line width=\linewidthothers}
    \addlegendentry{\acrshort{ppo}};
    \addlegendimage{C3, line width=\linewidthothers}
    \addlegendentry{\tppo};
    \addlegendimage{C5, line width=\linewidthothers}
    \addlegendentry{\acrshort{gsde}};
    \addlegendimage{C4, line width=\linewidthothers}
    \addlegendentry{\acrshort{sac}};    
    \addlegendimage{C6, line width=\linewidthothers}
    \addlegendentry{\acrshort{pink}};
        
    \end{axis}
\end{tikzpicture}

==> figure_and_table/hopper_jump/hopper_jump.tex <==
\begin{figure}[h!]    
    \hspace*{\fill}%
    \resizebox{0.9\textwidth}{!}{    
        \input{figure_and_table/hopper_jump/plot/legend}
    }% 
    \hspace*{\fill}%
    \newline
    \centering
    \hspace*{\fill}%
    \begin{subfigure}{0.32\textwidth}        
        \resizebox{\textwidth}{!}{\input{figure_and_table/hopper_jump/plot/height}}%
        \caption{Max Jump Height}
        \label{subfig:hopper_height_appendix}
    \end{subfigure}
    \hfill%       
    \begin{subfigure}{0.32\textwidth}        
        \resizebox{\textwidth}{!}{        
        \input{figure_and_table/hopper_jump/plot/to_goal}}%
        \caption{Distance to Goal}
        \label{subfig:hopper_goal}
    \end{subfigure}
    \hfill%       
    \begin{subfigure}{0.32\textwidth}        
        \resizebox{\textwidth}{!}{        
        \input{figure_and_table/hopper_jump/plot/reward}}%
        \caption{Overall, Height + Dist.}
        \label{subfig:hopper_reward}
    \end{subfigure}
    \hspace*{\fill}%    
    \caption{Hopper Jump\todo{name}}
    \label{fig:hopper_jump}
\end{figure}

==> figure_and_table/hopper_jump/plot/legend.tex <==
\begin{tikzpicture} 
\def\linewidthtcp{1mm}
\def\linewidthothers{0.5mm}

    \begin{axis}[%
    hide axis,
    xmin=10,
    xmax=50,
    ymin=0,
    ymax=0.4,
    legend style={
        draw=white!15!black,
        legend cell align=left,
        legend columns=-1, 
        legend style={
            draw=none,
            column sep=1ex,
            line width=1pt
        }
    },
    ]
    \addlegendimage{C0, line width=\linewidthtcp}
    \addlegendentry{\acrshort{tcp} (ours)};
    \addlegendimage{C1, line width=\linewidthothers}
    \addlegendentry{\acrshort{bbrl} Cov.};
    \addlegendimage{C9, line width=\linewidthothers}
    \addlegendentry{\acrshort{bbrl}};    
    \addlegendimage{C2, line width=\linewidthothers}
    \addlegendentry{\acrshort{ppo}};
    \addlegendimage{C3, line width=\linewidthothers}
    \addlegendentry{\acrshort{trpl}};
    \addlegendimage{C4, line width=\linewidthothers}
    \addlegendentry{\acrshort{sac}};    
    \addlegendimage{C5, line width=\linewidthothers}
    \addlegendentry{\acrshort{gsde}};
    \addlegendimage{C6, line width=\linewidthothers}
    \addlegendentry{\acrshort{pink}};
    
    
    
    % \addlegendimage{C6}
    % \addlegendentry{\acrshort{es}};

    
    % \addlegendimage{C4}
    % \addlegendentry{\acrshort{method-bb-ppo}};

    % \addlegendimage{C3}
    % \addlegendentry{\acrshort{method-bb} sparse};
    % \addlegendimage{C9}
    % \addlegendentry{\acrshort{method}};
    \end{axis}
\end{tikzpicture}

==> figure_and_table/list_of_symbols.tex <==
\renewcommand{\arraystretch}{1.33}
% \setlength{\aboverulesep}{0pt}
% \setlength{\belowrulesep}{0pt}
\begin{table}[htbp]
    \small
    \centering
    % \vspace{-0.7cm}
    \caption{List of symbols used in this paper.\vspace{0.2cm}}
    \begin{tabular}{cm{12.8cm}}
        \toprule
        \textbf{Symbol} & \textbf{Description}\\
        \hline
        $ a, ~\dot{a},~ \ddot{a} $ & One \acrshort{dof} trajectory position, velocity, and acceleration of a single time step respectively \\
        $ b $ & The time step of the initial conditions \\
        $ \mathcal{B} $ & Replay Buffer \\
        $ c $ & Coefficients of the general solutions of \acrshortpl{dmp}' \acrshort{ode} \\
        $ d,~D $ & Index and the number of \acrshortpl{dof} \\
        $ f $ & Forcing function of the original \acrshortpl{dmp} \\
        $ F $ & The source term in the \acrshortpl{dmp}'non-homogeneous \acrshortpl{ode} \\
        $ g $ & The Goal term of \acrshortpl{dmp} and \acrshortpl{pdmp}\\
        $ G $ & The return of RL\\
        % $ h $ &  \\
        $ \bm{H} $ & A combination of \acrshortpl{pdmp}' basis and boundary conditions terms, used in distribution computation \\
        $ i $ & index used in learning obj of MDP\\
        $ j,~J $ & index in N-step return importance sampling \\
        $ k, K $ & Index and the total number of the trajectory segments \\
        $ I $ & The two indefinite integrals in the closed form solution of \acrshortpl{dmp}' \acrshort{ode} \\
        $ \bm{l} $ & The length of a trajectory segment \\
        $ \bm{L} $ & The Cholesky decomposition of a covariance matrix \\
        $ L $ & Length of segment \\
        $ \mathcal{L} $ & The loss function to be minimized \\
        $ m, M $ & The index and number of basis functions and weights per \acrshortpl{dof}  \\
        $ N $ & The number of mini batch size  \\        
        $ \bm{o},~\mathcal{O} $ & Sensory observation and a set of observations \\
        $ p $ & probability \\
        $ Q $ & The state-action value function\\
        $ r $ & reward \\
        $ t, T $ & Index of time steps and the length of trajectory, i.e. the number of total time steps \\
        $ V $ & The state Value function\\
        $ \bm{w}, \bm{w_g} $ & The weights of \acrshortpl{dmp}, \acrshortpl{promp}, and \acrshortpl{pdmp}. A concatenation of weights and goal.\\
        $ x $ & The phase of the canonical system, which decays exponentially w.r.t time. \\        
        $ y $ & target values of the transformer critic \\           
        \midrule
        $ \alpha_x $ & Exponential decaying coefficient of the canonical system \\
        $ \alpha, \beta $ & Spring-damper coefficient of \acrshortpl{dmp}  \\
        $ \Delta  $ & The characteristic equation of \acrshortpl{dmp}' homogeneous \acrshortpl{ode}\\
        $ \epsilon $ & Gaussian white noise \\
        $ \theta $ & Neural Networks' learnable parameters \\
        $ \mu, \bm{\mu} $ & The mean of a certain probabilistic distribution \\
        $ \xi,~\bm{\xi} $ & One or multi time-step term determined by boundary conditions in \acrshortpl{pdmp}' trajectory computation \\
        % $ \pi $ &  \\
        $ \sigma^2 $ & The variance of a certain probabilistic distribution \\
        $ \bm{\Sigma} $ & The covariance of a certain probabilistic distribution \\
        $ \tau $ & Time scaling factor of \acrshortpl{dmp}, determining the execution speed \\
        $ \rho $ & Polyak rate \\
        $ \bm{\phi} $ & Critic Networks' learnable parameters \\
        $ \bm{\varphi} $ & Basis function forming up \acrshortpl{dmp}' forcing term \\
        $ \bm{\Phi} $ & Basis functions of one \acrshort{dof} used by \acrshortpl{promp} and \acrshortpl{pdmp}, written in matrix \\
        $ \bm{\Psi} $ & Blocked diagonal basis function matrix used by \acrshortpl{promp} and \acrshortpl{pdmp} for multi \acrshortpl{dof} trajectory \\
        $ \dot{\bm{\Phi}}, \dot{\bm{\Psi}} $ & Single and blocked diagonal velocity basis function matrices \\
        % $  $ &  \\
        \bottomrule
    \end{tabular}
     \vspace{-.5cm}
    \label{tab:model_comparison}
\end{table}
\renewcommand{\arraystretch}{1}

==> figure_and_table/meta50/backup.tex <==
\begin{figure}[b!]
    \hspace*{\fill}%
    \resizebox{0.8\textwidth}{!}{    
        \input{figure_and_table/meta50/legend_meta_50}
    }% 
    \hspace*{\fill}%
    \newline
    
  \centering
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_0.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_1.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_2.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_3.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_4.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_5.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_6.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_7.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_8.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_9.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_10.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_11.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_12.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_13.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_14.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
  \caption{Success Rate IQM of each individual Metaworld tasks.}
  \label{fig:your-label}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%     Page split     %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\begin{figure}[t!]
    \hspace*{\fill}%
    \resizebox{0.8\textwidth}{!}{    
        \input{figure_and_table/meta50/legend_meta_50}
    }% 
    \hspace*{\fill}%
    \newline
    
  \centering
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_15.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_16.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_17.pdf}
  \end{subfigure}
  \vspace{0.1cm}   
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_18.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_19.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_20.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_21.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_22.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_23.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_24.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_25.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_26.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_27.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_28.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_29.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_30.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_31.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_32.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
  \caption{Success Rate IQM of each individual Metaworld tasks.}
  \label{fig:your-label}
\end{figure}
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%     Page split 2   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\begin{figure}[t!]
    \hspace*{\fill}%
    \resizebox{0.8\textwidth}{!}{    
        \input{figure_and_table/meta50/legend_meta_50}
    }% 
    \hspace*{\fill}%
    \newline
    
  \centering
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_33.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_34.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_35.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_36.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_37.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_38.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_39.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_40.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_41.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_42.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_43.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_44.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_45.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_46.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_47.pdf}
  \end{subfigure}
  \vspace{0.1cm} 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_48.pdf}
  \end{subfigure}
  \begin{subfigure}{0.32\textwidth}
    \includegraphics[width=\linewidth]{figure_and_table/meta50/pdf_plots/plot_49.pdf}
  \end{subfigure}\hfill
  
  \vspace{0.1cm} 
  \caption{Success Rate IQM of each individual Metaworld tasks.}
  \label{fig:your-label}
\end{figure}
\afterpage{\newpage}

==> figure_and_table/target_options/target_options.tex <==
\begin{wraptable}{r}{0.5\textwidth}  % Adjust the width as needed
    \vspace{-3mm}
    \renewcommand{\arraystretch}{1.5}
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}
    \centering
    \caption{Options for the future return}
    \vspace{-2mm}
    \resizebox{0.5\textwidth}{!}{  % Resize to fit within the wrapfigure
        \begin{tabular}{ccc}
        \toprule
        \textbf{Option}& \textbf{Math}& \textbf{Description}\\
        \hline
        \textbf{V-target}& $V^{\text{tar}}_{\phi}(\vs_N)$ & State value after N steps\\
        \textbf{Q-target}& $Q^{\text{tar}}_{\phi}(\vs_N, \va_N, ...)$ & Action value after N steps\\
        \hline
        \textbf{Clipped}& $\text{Min}(\cdot, \cdot)$& Minimum of 2 target critics\\
        \textbf{Ensemble}& Avg.$(\cdot, \cdot) $& Mean of $\geq2$ target critics \\
        \bottomrule
        \end{tabular}
    }
    \label{tab:target_options}
    \renewcommand{\arraystretch}{1}
\end{wraptable} 
